Optical Magnetic Field Enhancement using Ultrafast Azimuthally Polarized Laser Beams and Tailored Metallic Nanoantennas

Structured light provides unique opportunities to spatially tailor the electromagnetic field of laser beams. This includes the possibility of a sub-wavelength spatial separation of their electric and magnetic fields, which would allow isolating interactions of matter with pure magnetic (or electric) fields. This could be particularly interesting in molecular spectroscopy, as excitations due to electric and -- usually very weak -- magnetic transition dipole moments can be disentangled. In this work, we show that the use of tailored metallic nanoantennas drastically enhances the strength of the longitudinal magnetic field carried by an ultrafast azimuthally polarized beam (by a factor of $\sim65$), which is spatially separated from the electric field by the beam's symmetry. Such enhancement is due to favorable phase-matching of the magnetic field induced by the electronic current loops created in the antennas. Our particle-in-cell simulation results demonstrate that the interaction of moderately intense ($\sim10^{11}$ W/cm$^2$) and ultrafast azimuthally polarized laser beams with conical, parabolic, Gaussian, or logarithmic metallic nanoantennas provide spatially isolated magnetic field pulses of several tens of Tesla.

==> figures_paper/GeometriesTable.tex <==
\begin{table}[b]
\caption{Shape definitions for the simulated antennas. The formulas for the calculation of the geometry-specific parameters are listed together with the propagation-axis dependent definition of the inner antenna radius $\rho\left(x\right)$. In the third column, the scanning parameters are provided.}
\label{tab:geometries}
\centering
\begin{tabular}{c|rp{0.01cm}l|c}
\hline
\multicolumn{1}{c}{Antennna type} &
\multicolumn{3}{c}{Formula} &
\multicolumn{1}{c}{Scan parameters} \\ \hline 
Cylindrical &\raggedright $\rho(x)$ &\centering=&\raggedleft$r_0$ & $L$  \\ \hline
Conical & $c_\textrm{c}$ &=&$\frac{x_\textrm{max}-x_\textrm{min}-L}{2}$   &  \\
 & $\rho(x)$ &=& $r_\textrm{max} - \frac{r_\textrm{max} - r_\textrm{min}}{L}\left(x-c_\textrm{c}\right)$ &  $r_\textrm{min}$, $r_\textrm{max}$  \\ \hline
 Parabola & $f$ &=& $\frac{r_\textrm{max}^2-r_\textrm{min}^2}{4L}$ &  -  \\
 & $c_\textrm{P}$ &=& $\frac{r_\textrm{max}^2}{4f}$ & - \\ 
 & $\rho(x)$ &=& $2\sqrt{f\cdot(x-c_\textrm{P})}$ & $r_\textrm{min}$, $L$, $\Delta L$  \\ \hline
 Gaussian &  $\sigma$ &=& $\frac{r_\textrm{max}}{2}$  &  -  \\
 & $c_\textrm{G}$ &=& $\frac{x_\textrm{max}-x_\textrm{min}-L}{2}$ &  - \\ 
 & $A$ &=& $\frac{r_\textrm{max}^2}{4f}$  &  - \\
 & $\rho(x)$ &=& $\sqrt{2\sigma^2\cdot\ln{\left(\frac{x-c_\textrm{G}}{A}\right)}}$ &$r_\textrm{min}$, $L$, $\Delta L$ \\ \hline
 Exponential & $c_\textrm{e}$ &=&$\frac{x_\textrm{max}-x_\textrm{min}-L}{2}$   &  \\
  & $\rho(x) $ &=& $ r_\mathrm{max}e^{-\kappa \left(x-c_\textrm{e}\right)}$ &  $\kappa$, $L$ \\ 
\end{tabular}
\end{table}

% \begin{table}[b]

% \begin{tabularx}{\textwidth}{XXXXXX}
% \multicolumn{2}{c}{Antennna type} &
% \multicolumn{2}{c}{Formula} &
% \multicolumn{2}{c}{Scan parameters}        \\ \hline

% \multicolumn{2}{c|}{
%     \begin{tabular}{l}
%     Cylindrical \\ 
%     Conical \\ 
%     Parabolic \\ 
%     {} \\
%     {} \\
%     Gaussian \\
%     {} \\
%     {} \\
%     {} \\
%     Exponential
%     \end{tabular}} 
% &
% \multicolumn{2}{c|}{
%     \begin{tabular}{r@{ = }l}
%     $\rho(x)$  & $r_0$ \\ 
%     $\rho(x)$  & $r_\textrm{max} - \frac{r_\textrm{max} - r_\textrm{min}}{L}x$ \\ 
%     $f$ & $\frac{r_\textrm{max}^2-r_\textrm{min}^2}{4L}$ \\
%     $c_\textrm{P}$ & $\frac{r_\textrm{max}^2}{4f}$ \\
%     $\rho(x)$ & $2\sqrt{f\cdot(x-c_\textrm{P})}$ \\
%     $\sigma$ & $\frac{r_\textrm{max}}{2}$ \\
%     $c_\textrm{G}$ & $\frac{x_\textrm{max}-x_\textrm{min}-L}{2}$ \\
%     $A$ & $\frac{r_\textrm{max}^2}{4f}$ \\
%     $\rho(x)$ & $\sqrt{2\sigma^2\cdot\ln{\left(\frac{x-c_\textrm{G}}{A}\right)}}$ \\
%     $\rho(x) $ & $ r_\mathrm{max}e^{-\kappa x}$
%     \end{tabular}} 
% &
% \multicolumn{2}{c|}{
%     \begin{tabular}{l}
%     $L$ \\
%     $r_\textrm{min}$, $r_\textrm{max}$ \\
%     - \\
%     - \\
%     $r_\textrm{min}$, $L$ \\
%     - \\
%     - \\
%     - \\
%     $r_\textrm{min}$, $L$, $\Delta L$ \\
%     $\kappa$, $L$ 
%     \end{tabular}} 
% \end{tabularx}
% \caption{}
% \label{tab:geometries}
% \end{table}




==> figures_paper/GeometriesTable_v1.tex <==
\begin{table}[b]
\centering
\begin{tabularx}{\textwidth}{YYY}
Antennna type                    & Formula                                                                 & Scan parameters      \\ \hline\hline
\multicolumn{1}{c|}{Cylindrical} & \multicolumn{1}{c|}{$\rho(x) = r_0$}                                    & $L$                  \\
\multicolumn{1}{c|}{Conical}     & \multicolumn{1}{c|}{$\rho(x) = r_\textrm{max} - \frac{r_\textrm{max} - r_\textrm{min}}{L}x$} & $r_\textrm{min}$, $r_\textrm{max}$ \\



\multicolumn{1}{c|}{Parabolic}   & \multicolumn{1}{c|}{$f = \frac{r_\textrm{max}^2-r_\textrm{min}^2}{4L}$}                         & -                 \\
\multicolumn{1}{c|}{}   & \multicolumn{1}{c|}{$c_\textrm{P} = \frac{x_\textrm{max}-x_\textrm{min}-L}{2}  - \frac{r_\textrm{max}^2}{4f}$}                         & -                  \\
\multicolumn{1}{c|}{}   & \multicolumn{1}{c|}{$\rho(x) = 2\sqrt{f\cdot(x-c)}$}                         & $r_\textrm{min}$, $L$                  \\

\multicolumn{1}{c|}{Gaussian}   & \multicolumn{1}{c|}{$\sigma = \frac{r_\textrm{max}}{2}$}                         & -                  \\
\multicolumn{1}{c|}{}   & \multicolumn{1}{c|}{$c_\textrm{G} = \frac{x_\textrm{max}-x_\textrm{min}-L}{2}$}                         & -                 \\
\multicolumn{1}{c|}{}   & \multicolumn{1}{c|}{$A = \frac{r_\textrm{max}^2}{4f}$}                         & -                  \\
\multicolumn{1}{c|}{}   & \multicolumn{1}{c|}{$\rho(x) = \sqrt{2\sigma^2\cdot\ln{\left(\frac{x-c}{A}\right)}}$}                         & $r_\textrm{min}$, $L$                  \\

\multicolumn{1}{c|}{Exponential} & \multicolumn{1}{c|}{$\rho(x) = r_0e^{-\kappa x}$}                        & $\kappa$, $L$       
\end{tabularx}
\caption{}
\label{tab:geometries}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[b]
\centering
\begin{tabularx}{\textwidth}{XXXXXX}
\multicolumn{2}{c}{Antennna type} &
\multicolumn{2}{c}{Formula} &
\multicolumn{2}{c}{Scan parameters}        \\ \hline

\multicolumn{2}{c|}{
    \begin{tabular}{l}
    Cylindrical \\ 
    Conical \\ 
    Parabolic \\ 
    {} \\
    {} \\
    Gaussian \\
    {} \\
    {} \\
    {} \\
    Exponential
    \end{tabular}} 
&
\multicolumn{2}{c|}{
    \begin{tabular}{r@{ = }l}
    $\rho(x)$  & $r_0$ \\ 
    $\rho(x)$  & $r_\textrm{max} - \frac{r_\textrm{max} - r_\textrm{min}}{L}x$ \\ 
    $f$ & $\frac{r_\textrm{max}^2-r_\textrm{min}^2}{4L}$ \\
    $c_\textrm{P}$ & $\frac{r_\textrm{max}^2}{4f}$ \\
    $\rho(x)$ & $2\sqrt{f\cdot(x-c_\textrm{P})}$ \\
    $\sigma$ & $\frac{r_\textrm{max}}{2}$ \\
    $c_\textrm{G}$ & $\frac{x_\textrm{max}-x_\textrm{min}-L}{2}$ \\
    $A$ & $\frac{r_\textrm{max}^2}{4f}$ \\
    $\rho(x)$ & $\sqrt{2\sigma^2\cdot\ln{\left(\frac{x-c_\textrm{G}}{A}\right)}}$ \\
    $\rho(x) $ & $ r_\mathrm{max}e^{-\kappa x}$
    \end{tabular}} 
&
\multicolumn{2}{c|}{
    \begin{tabular}{l}
    $L$ \\
    $r_\textrm{min}$, $r_\textrm{max}$ \\
    - \\
    - \\
    $r_\textrm{min}$, $L$ \\
    - \\
    - \\
    - \\
    $r_\textrm{min}$, $L$, $\Delta L$ \\
    $\kappa$, $L$ 
    \end{tabular}} 
\end{tabularx}
\caption{}
\label{tab:geometries}
\end{table}



==> figures_paper/GeometriesTable_v2.tex <==
\begin{table}[b]
\caption{Shape definitions for the simulated antennas. The formulas for the calculation of the geometry-specific parameters are listed together with the propagation-axis dependent definition of the inner antenna radius $\rho\left(x\right)$. In the third column, the scanning parameters are provided.}
\label{tab:geometries}
\centering
\begin{tabular}{c|rp{0.01cm}l|c}
\hline
\multicolumn{1}{c}{Antennna type} &
\multicolumn{3}{c}{Formula} &
\multicolumn{1}{c}{Scan parameters} \\ \hline 
Cylindrical &\raggedright $\rho(x)$ &\centering=&\raggedleft$r_0$ & $L$  \\ \hline
Conical & $\rho(x)$ &=& $r_\textrm{max} - \frac{r_\textrm{max} - r_\textrm{min}}{L}x$ &  $r_\textrm{min}$, $r_\textrm{max}$  \\ \hline
 & $f$ &=& $\frac{r_\textrm{max}^2-r_\textrm{min}^2}{4L}$ &  -  \\
Parabola & $c_\textrm{P}$ &=& $\frac{r_\textrm{max}^2}{4f}$ & - \\ 
 & $\rho(x)$ &=& $2\sqrt{f\cdot(x-c_\textrm{P})}$ & $r_\textrm{min}$, $L$, $\Delta L$  \\ \hline
  &  $\sigma$ &=& $\frac{r_\textrm{max}}{2}$  &  -  \\
Gaussian & $c_\textrm{G}$ &=& $\frac{x_\textrm{max}-x_\textrm{min}-L}{2}$ &  - \\ 
 & $A$ &=& $\frac{r_\textrm{max}^2}{4f}$  &  - \\
 & $\rho(x)$ &=& $\sqrt{2\sigma^2\cdot\ln{\left(\frac{x-c_\textrm{G}}{A}\right)}}$ &$r_\textrm{min}$, $L$, $\Delta L$ \\ \hline
 Exponential & $\rho(x) $ &=& $ r_\mathrm{max}e^{-\kappa x}$ &  $\kappa$, $L$ \\ 
\end{tabular}
\end{table}

% \begin{table}[b]

% \begin{tabularx}{\textwidth}{XXXXXX}
% \multicolumn{2}{c}{Antennna type} &
% \multicolumn{2}{c}{Formula} &
% \multicolumn{2}{c}{Scan parameters}        \\ \hline

% \multicolumn{2}{c|}{
%     \begin{tabular}{l}
%     Cylindrical \\ 
%     Conical \\ 
%     Parabolic \\ 
%     {} \\
%     {} \\
%     Gaussian \\
%     {} \\
%     {} \\
%     {} \\
%     Exponential
%     \end{tabular}} 
% &
% \multicolumn{2}{c|}{
%     \begin{tabular}{r@{ = }l}
%     $\rho(x)$  & $r_0$ \\ 
%     $\rho(x)$  & $r_\textrm{max} - \frac{r_\textrm{max} - r_\textrm{min}}{L}x$ \\ 
%     $f$ & $\frac{r_\textrm{max}^2-r_\textrm{min}^2}{4L}$ \\
%     $c_\textrm{P}$ & $\frac{r_\textrm{max}^2}{4f}$ \\
%     $\rho(x)$ & $2\sqrt{f\cdot(x-c_\textrm{P})}$ \\
%     $\sigma$ & $\frac{r_\textrm{max}}{2}$ \\
%     $c_\textrm{G}$ & $\frac{x_\textrm{max}-x_\textrm{min}-L}{2}$ \\
%     $A$ & $\frac{r_\textrm{max}^2}{4f}$ \\
%     $\rho(x)$ & $\sqrt{2\sigma^2\cdot\ln{\left(\frac{x-c_\textrm{G}}{A}\right)}}$ \\
%     $\rho(x) $ & $ r_\mathrm{max}e^{-\kappa x}$
%     \end{tabular}} 
% &
% \multicolumn{2}{c|}{
%     \begin{tabular}{l}
%     $L$ \\
%     $r_\textrm{min}$, $r_\textrm{max}$ \\
%     - \\
%     - \\
%     $r_\textrm{min}$, $L$ \\
%     - \\
%     - \\
%     - \\
%     $r_\textrm{min}$, $L$, $\Delta L$ \\
%     $\kappa$, $L$ 
%     \end{tabular}} 
% \end{tabularx}
% \caption{}
% \label{tab:geometries}
% \end{table}



